Designing Succinct Secondary Indexing Mechanism by Exploiting Column Correlations (Extended Version)

Database administrators construct secondary indexes on data tables to accelerate query processing in relational database management systems (RDBMSs). These indexes are built on top of the most frequently queried columns according to the data statistics. Unfortunately, maintaining multiple secondary indexes in the same database can be extremely space consuming, causing significant performance degradation due to the potential exhaustion of memory space. In this paper, we demonstrate that there exist many opportunities to exploit column correlations for accelerating data access. We propose HERMIT, a succinct secondary indexing mechanism for modern RDBMSs. HERMIT judiciously leverages the rich soft functional dependencies hidden among columns to prune out redundant structures for indexed key access. Instead of building a complete index that stores every single entry in the key columns, HERMIT navigates any incoming key access queries to an existing index built on the correlated columns. This is achieved through the Tiered Regression Search Tree (TRS-Tree), a succinct, ML-enhanced data structure that performs fast curve fitting to adaptively and dynamically capture both column correlations and outliers. Our extensive experimental study in two different RDBMSs have confirmed that HERMIT can significantly reduce space consumption with limited performance overhead in terms of query response time and index maintenance time, especially when supporting complex range queries.

==> meta.tex <==
%% ==================================================================
%% META REVIEWER
%% ==================================================================

\separator
\metareviewer

\commentx{D1,D2}{Add experiments depending on what is claimed as novelty. 
For instance, if claimed novelty is equi-depth mapping instead of equi-width mapping, 
there should be a realistic experiment to verify the benefit.
If claimed novelty is the data structure to maintain the mapping, 
there should be lookup/maintenance overhead comparison to plain indexes simply storing 
from-bucket-ID and to-bucket-IDs.\isslabel{RM.D1D2}}

From a high level, the novelty of \system lies in that it is a \textit{\textbf{succinct}, \textbf{ML-enhanced}, and \textbf{tree-structured} index, which \textbf{adaptively} and \textbf{dynamically} captures \textbf{complex correlations} with \textbf{outlier handling} to accelerate unindexed column accesses.}

%From a high level, \system's novelty is that \textit{it employs a novel \textbf{ML-enhanced tree structure} to 
%\textbf{adaptively} and \textbf{dynamically} capture 
%\textbf{complex correlations} and \textbf{outliers} to accelerate unindexed column accesses.}

\vspace{2.5mm}

While both \system's \tree and Correlation Maps (CM) attempt to leverage column correlations to 
accelerate access to unindexed columns, they are different in many aspects. 
We list the similarities and differences below.


\underline{Similarities:}

\begin{itemize}[noitemsep,topsep=0pt]
  \item \tree and CM both leverage column correlations to produce compressed access methods for unindexed columns.
\end{itemize}

\underline{Differences:}

\begin{itemize}[noitemsep,topsep=0pt]
  \item \tree is an \textbf{ML-enhanced} and \textbf{tree-structured} index, and it greatly reduces storage consumption
  by summarizing correlations using tiny linear regression models. In contrast, CM adopts a map-like structure. It physically stores the bucket mappings between correlated columns;
  %and consequently consume more space than \tree;
  \item \tree not only captures correlations using tiered curve fitting but also \textbf{handles outliers}. This makes 
  \tree robust to noisy data which is prevalent in real-world applications. In contrast, CM does not include 
  any specific scheme to handle outliers, and hence its performance can drop when confronting sparsely distributed noisy data;
  \item \tree \textbf{adaptively} constructs its internal structures
  and \textbf{automatically} decides the partition granularity based on the tree structure properties and parameters.
  In comparison, CM relies on its tuning advisor to decide the granularity for its single-layer buckets by building multiple histograms beforehand;
  \item \tree \textbf{dynamically} maintains its internal structures, and performs \textbf{on-demand} reorganization 
  to re-optimize its performance in the presence of large amounts of insert/delete/update operations. Although CM supports insertions and deletions, it is unknown how 
  CM adapts to dynamic workload where the underlying data drastically changes over time;
  \item \system is a \textbf{general} secondary indexing mechanism and can exploit multiple correlations on the same table. In contrast, 
  CM can only exploit correlations when there is a clustered index on the host column, and there can be at most one clustered index on any single table;
  \item \system can function efficiently in both \textbf{main-memory} and \textbf{disk-based} RDBMSs, as demonstrated by our empirical study, whereas CM's cost model is specifically designed for disk-based RDBMSs;
  \item \system is specifically designed for many-valued numerical data columns. Its \tree partitions key space on demand, and uses ML models to summarize correlations
  with minimal space consumption. Although CM can work for many-valued numerical data columns, %categorical data columns,
  % works best when the number of distinct values for each column is small (typical for categorical data columns). 
  it resorts to bucketing the column ranges when handling columns with a large number of distinct values. It adopts a sophisticated CM advisor to analyze the best bucketing strategy in order to trade off 
  between space and efficiency.
  % However, a sophisticated CM advisor needs to analyze, ahead of time, how to bucket the correlated columns, in order to trade off between space and efficiency. The \tree structure in \system does not suffer from this problem, since we utilize ML models to capture correlation. 
  For columns with a huge number of distinct values, if there is a strong correlation between the two columns, \tree can still use a very small number of tree nodes with very small sized outlier buffers. In the presence of a perfect linear correlation, \tree just needs a single tree node to capture the correlation.
\end{itemize}

\vspace{2.5mm}


\system's \tree design is orthogonal to ``equi-depth'' (i.e., partition based on tuple count) or ``equi-width'' (i.e., 
partition based on value range) mapping. 
While Figure 2 in our paper demonstrated a ``equi-width'' mapping scheme\footnote{We find that 
the reviewers may interpret ``equi-width'' differently. In most RDBMSs, 
``equi-width'' refers to value-range based partition. See \url{https://www.postgresql.org/docs/11/functions-math.html}.}, \tree can naturally support ``equi-depth''
mapping, by either sorting the target column beforehand\footnote{We actually implemented this scheme 
in an early version of \tree.} or sampling and building histograms on the target columns ahead of time, which is also required by CM. This process does incur some extra overhead, thus we prefer the ``equi-width'' approach. 

\tree serves the incoming queries by applying the generated linear functions rather than chasing the stored pointers,
hence it does not store any ``from-bucket-IDs''\footnote{We interpret ``from-bucket-IDs'' as the 
ID of the bucket in the target column (or the unclustered column mentioned in the CM paper).} information. 
This actually leads to a big save in space consumption, as \tree does not need to maintain many-to-many 
mappings among buckets.

% In the revision, we added a new experiment to compare index lookup/maintenance overhead in comparison to CM.

Based on the reviewers' suggestions, we have revised our paper to highlight the novelties of our approach (see Section 1, Section 8, 
and Appendix C). 
To better justify our claims, we have also added more experiments to
measure \tree's overhead in lookups and structure maintenance (see Section 7.3 and Section 7.7), and compared it with CM (see Appendix C and Appendix E).
Please refer to \issref{RM.D4}{RM.D4} for more discussion.
 % We modified our novelty claim in Introduction section and put a more clear statement: our work advocates a novel tree structure that leverages tiered curve fitting to model the complex correlations. We also added an experiment to compare \system against a CM prototype. Please refer to \issref{R1.W1}{R1.W1} and \issref{R1.W2}{R1.W2} for more details.


\commentx{D3}{What kinds of correlations in real world can be exploited by each approach? 
Equi-depth vs equi-width is one. What else, and how often is it observed in real world? 
This is harder to set up as an experiment because "real workload/dataset" is a very vague/subjective matter. 
But getting real world data to back up any claims would be a great step.}

``Equi-depth'' and ``equi-width'' are just two different methods that data are partitioned for the construction of \tree or the bucketization of CM. As discussed in \issref{RM.D1D2}{RM.D1D2}, \system's \tree design can support both
partition methods, although the ``equi-width'' approach is preferred in \system due to performance reasons. We believe this is an orthogonal issue to the exploitation of correlations in real world.

Correlations can exist in both categorical and numerical data columns. 
\system is specifically tailored for exploiting correlations among numerical data columns.
Typical examples include package delivery (ship date v.s. receipt date),
transportation (ticket fare v.s. distance), investment (revenue v.s. profit), 
and many other applications as mentioned in our paper.
Mainstream commercial RDBMSs 
(e.g., Oracle~\cite{oracle-correlation}, IBM Db2~\cite{db2-correlation}, Microsoft SQL Server~\cite{sqlserver-correlation}) 
can automatically detect and exploit these correlations for optimization purpose.
In fact, DBA can also manually identify correlations for RDBMSs.
For example, 
Microsoft SQL Server supports \texttt{DATE\_CORRELATION\_OPTIMIZATION} option to exploit correlations 
between two datetime columns~\cite{sqlserver-correlation}.

% As discussed in \issref{RM.D1D2}{RM.D1D2}, CM works best when the number of distinct values for both host and target columns are small, typical for categorical data columns, while \system's strength is in supporting numerical data columns. 
% Correlations in numerical columns are prevalent in real-world applications. Correlations on date and time columns (e.g. order date vs. due date and ship date vs. receipt date) are so common in many application domains that 
% Microsoft SQL Server introduced a special DATE\_CORRELATION\_OPTIMIZATION database option just to exploit such correlations for query processing~\cite{sqlserver-correlation}. Other common examples include transportation (ticket fare v.s. distance), investment (revenue v.s. profit), 
% and many other applications as mentioned in our paper. In fact, such correlations are not only studied in research papers 
% and system prototypes, but also widely exploited in many
% the mainstream commercial RDBMSs 
% (e.g., Oracle~\cite{oracle-correlation}, IBM Db2~\cite{db2-correlation}, Microsoft SQL Server~\cite{sqlserver-correlation}) for optimization purpose.

% In terms of real world datasets that exhibit correlations on some columns, we experimented with three such datasets in our paper. The CM paper also included two other real world datasets.

%We believe that ``equi-depth'' and ``equi-width'' are not quite relevant to the 
%column correlation modeling and discovery
%discussed in our paper.
%In the context of classic RDBMSs, ``equi-depth'' (i.e., partition based on tuple count) and 
%``equi-width'' (i.e., partition based on value range) are different schemes the optimizer adopts to build
%histograms. \system does not rely on any pre-built histograms to build \tree. 
%Also, as discussed in \issref{RM.D1D2}{RM.D1D2}, \system's \tree design can support both
%``equi-depth'' and ``equi-width'' partitions, but for performance reason, it partitions column space based 
%on value range.

% Column correlations are prevalent in real-world applications, 
%Column correlations can exist in both categorical and numerical data columns.
%\system is not designed for categorical columns. Instead, 
%it is specifically tailored for high cardinality, numerical data columns.
%Correlations in numerical columns are prevalent in real-world applications. 
%Typical examples include package delivery (ship date v.s. receipt date),
%transportation (ticket fare v.s. distance), investment (revenue v.s. profit), 
%and many other applications as mentioned in our paper.
%In fact, such correlations are not only used in research papers 
%and system prototypes, but also widely exploited in \textbf{almost all} 
%the mainstream commercial RDBMSs 
%(e.g., Oracle, IBM Db2, Microsoft SQL Server) for 
%query/storage optimization purpose.


%The applications used in our paper are real, and actually they are very representative.
%Recall that \system relies on the RDBMSs' optimizers to recommend correlations. 
%Typically, commercial RDBMSs measure and recommend correlations using different 
%coefficients, including \textit{Pearson coefficient} and \textit{Spearman coefficient}.
%The applications used in our paper can essentially cover cases detected 
%by both coefficients.
%Specifically, \textsc{Synthetic-Linear} and \textsc{Stock} contain linear correlation, 
%which can be detected using Pearson coefficient; 
%\textsc{Synthetic-Sigmoid} and \textsc{Sensor} contain non-linear 
%correlation, which can be detected using Spearman coefficient.
%In our experiment, we also changed the percentage of data noises to control 
%the correlation.




The applications used in our paper are very representative, and can actually cover cases 
detected by both \textit{Pearson coefficient} and \textit{Spearman coefficient}, 
the two typical coefficients used in many commercial RDBMSs (see \issref{R2.D3}{R2.D3} for detailed discussion).
Specifically, \textsc{Synthetic-Linear} and \textsc{Stock} contain linear correlation, 
which can be detected using Pearson coefficient; 
\textsc{Synthetic-Sigmoid} and \textsc{Sensor} contain non-linear 
correlation, which can be detected using Spearman coefficient.


Based on the reviewers' suggestions, we have expanded our discussion on 
the correlation types and further described how existing commercial 
RDBMSs detect and exploit column correlations.
We also used the Dow-Jones and S\&P 500 example to better explain how \system 
works in real-world data.
Please refer to Section 7.2, Appendix A, and Appendix D.1 for more discussion.

% Please refer to \issref{R2.D3}{R2.D3} for more discussion.


% To better back up our claims, we have added more detailed analysis on our real-world applications (see Section 8 and Appendix E). 
% Please refer to \issref{RM.D7}{RM.D7} and ?????? for more discussion.






\commentx{D4}{Review the high-level statement of novelty w.r.t. CM. ("However, this solution cannot model complex correlations,
and can suffer from significant performance drop when handling continuous and high cardinality numerical data.") If
you stand by this statement, you should explain intuitively why CM does poorly in these cases, and what feature of
your solution makes it do better. We would like to see both detailed textual explanation in addition to detailed
experimental evidence in support. If you choose to modify this statement, that's OK too, again providing text and
experiments to justify the new claim.\isslabel{RM.D4}}

We agree that this statement is too vague and was not well supported with experimental evidence. 
To address this issue, 
we have implemented the CM method and compared it with \system.

% \system can outperform CM in many cases. To confirm this statement, we have added several experiments to empirically 
% compare \system and CM. 

Please note that, since we \textbf{cannot} find any publicly available implementation of CM, 
we implemented CM on our own.
The original design of CM \textbf{cannot} exploit correlations between two unclustered columns,
and it is unknown how its cost model can work in main-memory RDBMSs. 
We hence made essential modifications to the original design of CM to make it comparable with \system.
Specifically, as the host index in our context is not necessarily a clustered index, CM has to delay the 
false positive removal to base table validation phase (see Step 4 in Section 5.2); 
CM relies on ``CM Advisor'' to perform data sampling and build multiple histograms in order to obtain 
best bucketing scheme. To ensure that our CM implementation can achieve its optimal performance, 
we do not build ``CM Advisor''. Instead, we perform \textit{brute-force} experiments and do parameter 
sweeping to test CM's performance with various types of bucketing schemes. 


The main observation from our experiments is that \system saves more storage space, 
and can outperform CM in many cases, especially in the presence of noisy data.
This is because \system summarizes correlation in tiny linear regression models, 
and provide outlier handling mechanism to identify and maintain outliers.
In contrast, CM has to physically store and lookup mappings, and the absence 
of outlier handling scheme in CM can yield high false positive rate when performing 
lookups.

More than comparing CM with \system, we also analyzed CM's behaviors in main-memory RDBMSs. 
Different from the disk-based RDBMS scenarios, increasing CM's bucket size does not 
necessarily decrease the performance. This is because main-memory RDBMSs maintain 
primary/secondary indexes as well as base tables in memory, and CM's standalone lookup performance 
becomes more critical. While increasing the bucket size may increase false positive rate 
(but this is not necessarily true when noisy data exists), CM's standalone performance is also improved.
As a result, the overall lookup performance will be affected by both factors.
Hence, we conclude that tuning CM in main-memory scenario becomes more challenging.

We have reported the experiment results as well as the corresponding findings in the revised version of our paper (see Appendix E).

\commentx{D5}{Overall there seem to be many missing details in the presentation with regards to the data structure. 
These should be presented in detail.}

Based on the reviewers' suggestions, we have added more descriptions on 
correlation discovery, index reorganization, parameter tuning and space-compute tradeoff in the 
revised version of our paper.
Please refer to Responses to Reviewers 2,3,4 for detailed discussion.

\commentx{D6}{Add discussion on how memory usage trades off with computation.}

Based on the reviewers' suggestions, we have expanded the discussion 
on the tradeoff between memory usage and computation and added a set 
of experiment to confirm our claims (see Section 6 and Section 7.3).
Please refer to Responses to Reviewers 2,3,4 for detailed discussion.

\commentx{D7}{Show results and discussion on cases where correlations do not always have good properties 
such as bounding of difference.}

Based on the reviewers' suggestions, we have expanded the discussion 
on how \system handles cases where bounding of difference does not exist.% and how \system handles outliers.
% Please refer to 
Please refer to Responses to Reviewers 2,3,4 for detailed discussion.
 % to learn more details about how to discover good correlations for \system and \issref{R4.D2b}{R4.D2b} for the explanation of bounded differences.


